PolyMorph: Increasing P300 Spelling Efficiency by Selection Matrix Polymorphism and Sentence-Based Predictions

P300 is an electric signal emitted by brain about 300 milliseconds after a rare, but relevant-for-the-user event. One of the applications of this signal is sentence spelling that enables subjects who lost the control of their motor pathways to communicate by selecting characters in a matrix containing all the alphabet symbols. Although this technology has made considerable progress in the last years, it still suffers from both low communication rate and high error rate. This article presents a P300 speller, named PolyMorph, that introduces two major novelties in the field: the selection matrix polymorphism, that reduces the size of the selection matrix itself by removing useless symbols, and sentence-based predictions, that exploit all the spelt characters of a sentence to determine the probability of a word. In order to measure the effectiveness of the presented speller, we describe two sets of tests: the first one in vivo and the second one in silico. The results of these experiments suggest that the use of PolyMorph in place of the naive character-by-character speller both increases the number of spelt characters per time unit and reduces the error rate.

==> invitro_results.tex <==
%!TEX root = main.tex

\subsection{\emph{In-silico}}

\pgfplotstableread{
Lang	Time_nKB	C_nKB	W_nKB	S_nKB	MTC_nKB	MTW_nKB	MTS_nKB	CPM_nKB	WPM_nKB	SPM_nKB	Time_KB	C_KB	W_KB	S_KB	MTC_KB	MTW_KB	MTS_KB	CPM_KB	WPM_KB	SPM_KB	Time_P3S	C_P3S	W_P3S	S_P3S	MTC_P3S	MTW_P3S	MTS_P3S	CPM_P3S	WPM_P3S	SPM_P3S
English	24937550.125	1104177	180161	10000	22.585	138.418	2493.755	2.66	0.43	0.02	11515342.250	1166867	189938	10000	9.869	60.627	1151.534	6.08	0.99	0.05	46513456.125	1104177	180161	10000	42.125	258.177	4651.346	1.42	0.23	0.01
German	21477311.000	1015970	137598	10000	21.140	156.087	2147.731	2.84	0.38	0.03	8691222.875	1021348	137450	10000	8.510	63.232	869.122	7.05	0.95	0.07	42797736.250	1015970	137598	10000	42.125	311.035	4279.774	1.42	0.19	0.01
French	25375109.500	1183358	185089	10000	21.443	137.097	2537.511	2.80	0.44	0.02	9881060.500	1055790	166292	10000	9.359	59.420	988.106	6.41	1.01	0.06	49848955.750	1183358	185089	10000	42.125	269.324	4984.896	1.42	0.22	0.01
Italian	25516760.000	1132476	172385	10000	22.532	148.022	2551.676	2.66	0.41	0.02	9539286.625	1011753	154604	10000	9.428	61.701	953.929	6.36	0.97	0.06	47705551.500	1132476	172385	10000	42.125	276.738	4770.555	1.42	0.22	0.01
Finnish	19689547.500	898813	102291	10000	21.906	192.486	1968.955	2.74	0.31	0.03	6961666.500	875585	99874	10000	7.951	69.704	696.167	7.55	0.86	0.09	37862497.625	898813	102291	10000	42.125	370.145	3786.250	1.42	0.16	0.02
Hungarian	15148221.625	914398	146779	10000	16.566	103.204	1514.822	3.62	0.58	0.04	9184826.375	953824	151024	10000	9.629	60.817	918.483	6.23	0.99	0.07	38519015.750	914398	146779	10000	42.125	262.429	3851.902	1.42	0.23	0.02
{Italian Curated}	8000037.250	356238	55005	10000	22.457	145.442	800.004	2.67	0.41	0.07	4646009.250	383541	59631	10000	12.113	77.913	464.601	4.95	0.77	0.13	15006525.750	356238	55005	10000	42.125	272.821	1500.653	1.42	0.22	0.04

}\insilicodata

\pgfplotstableread{
Lang	Time_nKB	C_nKB	W_nKB	S_nKB	MTC_nKB	MTW_nKB	MTS_nKB	CPM_nKB	WPM_nKB	SPM_nKB	Time_KB	C_KB	W_KB	S_KB	MTC_KB	MTW_KB	MTS_KB	CPM_KB	WPM_KB	SPM_KB	Time_P3S	C_P3S	W_P3S	S_P3S	MTC_P3S	MTW_P3S	MTS_P3S	CPM_P3S	WPM_P3S	SPM_P3S
English	37921461.250	1104177	180161	10000	34.344	210.487	3792.146	1.75	0.29	0.02	39828620.250	1166867	189938	10000	34.133	209.693	3982.862	1.76	0.29	0.02	46513456.125	1104177	180161	10000	42.125	258.177	4651.346	1.42	0.23	0.01
German	32043448.500	1015970	137598	10000	31.540	232.877	3204.345	1.90	0.26	0.02	31964631.500	1021348	137450	10000	31.297	232.555	3196.463	1.92	0.26	0.02	42797736.250	1015970	137598	10000	42.125	311.035	4279.774	1.42	0.19	0.01
French	38984989.750	1183358	185089	10000	32.944	210.628	3898.499	1.82	0.28	0.02	34868144.375	1055790	166292	10000	33.026	209.680	3486.814	1.82	0.29	0.02	49848955.750	1183358	185089	10000	42.125	269.324	4984.896	1.42	0.22	0.01
Italian	37166896.625	1132476	172385	10000	32.819	215.604	3716.690	1.83	0.28	0.02	33281607.750	1011753	154604	10000	32.895	215.270	3328.161	1.82	0.28	0.02	47705551.500	1132476	172385	10000	42.125	276.738	4770.555	1.42	0.22	0.01
Finnish	25333221.000	875585	99874	10000	28.933	253.652	2533.322	2.07	0.24	0.02	29092310.875	914398	146779	10000	31.816	198.205	2909.231	1.89	0.30	0.02	36884018.125	875585	99874	10000	42.125	369.306	3688.402	1.42	0.16	0.02
Hungarian	30207438.250	953824	151024	10000	31.670	200.017	3020.744	1.89	0.30	0.02	11499202.125	356238	55005	10000	32.280	209.057	1149.920	1.86	0.29	0.05	40179836.000	953824	151024	10000	42.125	266.049	4017.984	1.42	0.23	0.01
{Italian Curated}	11499202.125	356238	55005	10000	32.280	209.057	1149.920	1.86	0.29	0.05	12394496.500	383541	59631	10000	32.316	207.853	1239.450	1.86	0.29	0.05	15006525.750	356238	55005	10000	42.125	272.821	1500.653	1.42	0.22	0.04

}\insilicodatanohints

\pgfplotsset{unit code/.code={\si{#1}}}

PolyMorph reduces the absolute redundancy of the channel code in a significant way with respect to P3Speller for all the considered languages ($\mu=0.93$, $\sigma=0.11$ smaller than $\mu=4.13$, $\sigma=0.13$, Wilcoxon test: $V = 28$, $p$-value $=0.007813$), but  
the amplitude does not depend in a substantial way on the language itself. 
The AR reduction affects ISR which is also decreased. However, due to the prediction characters introduced in PolyMorph, this contraction becomes evident exclusively 
when the sentence to be spelt is not present in the KB (see Tables~\ref{table:invivo_ISR} and~\ref{table:ISR}). As the matter of facts, 
Wilcoxon test revealed a significant reduction in ISR when using PolyMorph in place of P3Speller in such a case ($\mu=11.22$, $\sigma=0.37$ smaller than $\mu=12.00$, $\sigma=0.00$,  Wilcoxon test: $V = 28$, $p$-value $=0.007813$). 
On contrary, the same test does not highlight differences between PolyMorph and P3Speller in ISR when the spelt sentence is contained in the KB ($\mu=12.42$, $\sigma=0.57$ vs $\mu=12.00$, $\sigma=0.00$,  Wilcoxon test: $V = 24$, $p$-value $=0.05384$ ), 
but it tops again P3Speller if we take into account the additional prediction row ($\mu=13.00$, $\sigma=0.00$ for P3Speller with an additional row, Wilcoxon test: $V = 28$, $p$-value $= 0.01113$). 

PolyMorph exhibits an increased OCM with respect to P3Speller whether the spelt sentences are contained into the KB ($\mu=6.38$, $\sigma=0.81$ greater than  
$\mu=1.43$, $\sigma=0.00$, Wilcoxon test: $V = 28$, $p$-value $=0.007813$) or not 
 ($\mu=2.86$, $\sigma=0.35$ greater than  $\mu=1.43$, $\sigma=0.00$, Wilcoxon test: $V = 28$, $p$-value $=0.01113$ ). 
With no doubt, the former case is the most favorable one as it causes a mean improvement of about $350\%$ with respect to P3Speller, but the latter case has a still remarkable mean enhancement of about $100\%$ (see Table~\ref{table:charmin}).  
The amplitude of the improvement depends, as expected, on the user language with peaks of about $430\%$ for Finnish $\Ain$ (former case) and $150\%$ for spelling Hungarian $\Aout$ (latter case). 
Intriguingly, there is no apparent relation between the OCM gain in spelling either $\Ain$'s  or $\Aout$'s  (i.e., sentences in the KB and sentences outside the KB) ($\chi$-test: $\chi=0.34$, $p$-value$=1.0$). 
As concern the former condition test set, the worst case language appears to be the one of the 
Italian curated phrasebook. This is due to the sentence lengths in the phrasebooks: 
since the sentences in the Italian curated phrasebook are shorter on average than those in the other 
phrasebooks (see Table~\ref{table:statistics}), the effectiveness of the SSP based 
prediction is reduced. 

The data obtained when predictions were disabled highlighted that 
most of the PolyMorph speed-up is due to the predictions themselves. However,  
the only adoption of a ``compressed'' channel code together with the matrix polymorphism 
increased OCM significantly with 
respect to P3Speller OCM in spelling both $\Aout$ ($\mu=1.88$, $\sigma=0.10$ greater than $\mu=1.43$, $\sigma=0.00$, Wilcoxon test: $V = 28$, $p$-value $=0.007813$)  and 
$\Ain$ ($\mu=1.85$, $\sigma=0.05$ greater than $\mu=1.43$, $\sigma=0.00$, Wilcoxon test: $V = 28$, $p$-value $=0.007813$).  
%and the enhancement goes from the $23\%$ (English $\Aout$) to the $46\%$ (Finnish $\Aout$).

While the use of PolyMorph in place of P3Speller increases OCM,  SM drop from a mean of $\mu=1.43$ ($\sigma=0.0$) to $\mu=1.29$ ($\sigma=0.03$), in spelling sentences that are not contained in the KB, and 
and to $\mu=1.20$ ($\sigma=0.04$), in spelling sentences that are in the KB. No substantial differences in spelling either $\Aout$'s or $\Ain$'s have been highlighted ($\chi$-test: $\chi=0.34$, $p$-value$=1.0$). 


\begin{table}
\begin{center}
\begin{tabular}{lccccccccccc}
\toprule
\headcol & \multicolumn{3}{c}{P3Speller}& &\multicolumn{3}{c}{PolyMorph - Pred.} & &\multicolumn{3}{c}{PolyMorph - No Pred.}\\
 \rulefiller\cmidrule(r){2-4} \cmidrule(r){6-8}\cmidrule(r){10-12}
\headcol Lang&$\arate>$&$\irate[1000]$&$\oAR[1000] $&&$\arate[1000]$&$\irate[1000]$&$\AR[1000]$&&$\arate[1000]$&$\irate[1000]$&$\AR[1000]$\\
\midrule
\English&$4.95$&$0.97$&$3.98$&&$4.85$&$4.01$&$0.84$&&$4.85$&$4.30$&$0.29$\\
\rowcol \German&$4.95$&$0.80$&$4.15$&&$4.82$&$3.91$&$0.91$&&$4.82$&$4.23$&$0.32$\\
\French&$4.95$&$0.85$&$4.10$&&$4.82$&$3.95$&$0.87$&&$4.82$&$4.26$&$0.31$\\
\rowcol \Italian&$4.95$&$0.81$&$4.14$&&$4.81$&$3.99$&$0.83$&&$4.81$&$4.26$&$0.28$\\
\Finnish&$4.95$&$0.73$&$4.22$&&$4.79$&$3.82$&$0.96$&&$4.79$&$4.21$&$0.39$\\
\rowcol \Hungarian&$4.95$&$0.63$&$4.32$&&$4.77$&$3.81$&$0.97$&&$4.77$&$4.19$&$0.38$\\
\ItalianC&$4.95$&$0.98$&$3.97$&&$4.73$&$3.60$&$1.13$&&$4.73$&$4.13$&$0.52$\\
\bottomrule
\end{tabular}
\caption{Channel code entropies and absolute redundancy.  
%$R$  denotes the absolute rate of the P3Speller channel code and it is computed as $\log{|\Sigma|}$, where $\Sigma$ is the set of symbols in 
%the selection matrix. Since the latin alphabet includes 27 characters and we have 4 mandatory symbols, $|\Sigma|$ is greater than $31$ 
%and $R$ is lower bounded by $\log{31}\approx 4.95$. 
%The columns $\AR[1000]$ and $\oAR[1000]$ report, for each channel code, the absolute redundancy approximations $\arate[1000]-\irate[1000]$ and $\arate-\irate[1000]$, respectively. 
%Notice that, by 
By removing predictions, we could reduce the absolute redundancy of the PolyMorph channel code, however, this choice would reduce 
the speller efficiency (e.g., see Table~\ref{table:charmin}).%the differences between Figure~\ref{fig:insilico:spelling_time1} and \ref{fig:insilico:spelling_time1_no_hints}).
}\label{table:rate_and_redundancy} 
\end{center}
\end{table}



\pgfplotstableread{
Lang	P3S	PM_Pred_Out	PM_Pred_In	PM_no_Pred_Out	PM_no_Pred_In
English	12.00	11.70	12.81	10.58	10.55
German	12.00	11.34	12.77	10.41	10.40
French	12.00	11.47	12.85	10.35	10.38
Italian	12.00	11.40	12.77	10.30	10.31
Finnish	12.00	10.81	12.48	9.78	9.78
Hungarian	12.00	11.18	11.80	10.40	10.35
{Italian Curated}	12.00	10.66	11.44	9.92	9.92

}\insiliconis

\begin{figure}
\begin{center}
\begin{tikzpicture}[scale=0.80]
\begin{axis}
[
width=18cm,
height=6cm,
ymajorgrids,
ybar,
ymode = log,
xlabel = Language,
nodes near coords, 
every node near coord/.append style={rotate=-90, anchor=east},
%symbolic x coords={Danish,English,Finnish,French,German,Hungarian,Italian},
%xtick={Danish,English,Finnish,French,German,Hungarian,Italian},
symbolic x coords={English,German,French,Italian,Finnish,Hungarian,{Italian Curated}},
xtick={English,German,French,Italian,Finnish,Hungarian,{Italian Curated}},
ylabel style={align=center}, 
ylabel=Intensifications per\\Selection and Repetition,
ymin = 0,
ymax=13.8,
%ymax=2600,     
%y unit=\si{\second},
%max space between ticks=30pt, 
%ytick={700,1400,2100},
legend columns=-1,
legend style={/tikz/every even column/.append style={column sep=0.3cm},at={(0.5,-0.3)}, anchor=north},
point meta=rawy,
%scaled y ticks=false,
%yticklabel style={
%            /pgf/number format/.cd,
%            sci,
%            sci generic={mantissa sep=\times,exponent={10^{#1}}}
%            }
]
\addplot[P3SpellerColor,fill=P3SpellerColor] table[y=P3S] from \insiliconis;
\addlegendentry{P3Speller};
\addplot[nKBColor,fill=nKBColor] table[y=PM_Pred_Out] from \insiliconis;
\addlegendentry{PolyMorph - $\Aout$};
\addplot[KBColor,fill=KBColor] table[y=PM_Pred_In] from \insiliconis;
\addlegendentry{PolyMorph - $\Ain$};
\end{axis}
\end{tikzpicture}
\caption{ .}\label{fig:insilico:ISR_Pred}
\end{center}
\end{figure}




\begin{figure}
\begin{center}
\begin{tikzpicture}[scale=0.80]
\begin{axis}
[
width=18cm,
height=6cm,
ymajorgrids,
ybar,
ymode = log,
xlabel = Language,
nodes near coords, 
every node near coord/.append style={rotate=-90, anchor=east},
%symbolic x coords={Danish,English,Finnish,French,German,Hungarian,Italian},
%xtick={Danish,English,Finnish,French,German,Hungarian,Italian},
symbolic x coords={English,German,French,Italian,Finnish,Hungarian,{Italian Curated}},
xtick={English,German,French,Italian,Finnish,Hungarian,{Italian Curated}},
ylabel style={align=center}, 
ylabel=Intensifications per\\Selection and Repetition,
ymin = 0,
ymax=13,
%ymax=2600,     
%y unit=\si{\second},
%max space between ticks=30pt, 
%ytick={700,1400,2100},
legend columns=-1,
legend style={/tikz/every even column/.append style={column sep=0.3cm},at={(0.5,-0.3)}, anchor=north},
point meta=rawy,
%scaled y ticks=false,
%yticklabel style={
%            /pgf/number format/.cd,
%            sci,
%            sci generic={mantissa sep=\times,exponent={10^{#1}}}
%            }
]
\addplot[P3SpellerColor,fill=P3SpellerColor] table[y=P3S] from \insiliconis;
\addlegendentry{P3Speller};
\addplot[nKBColor,fill=nKBColor] table[y=PM_no_Pred_Out] from \insiliconis;
\addlegendentry{PolyMorph - $\Aout$};
\addplot[KBColor,fill=KBColor] table[y=PM_no_Pred_In] from \insiliconis;
\addlegendentry{PolyMorph - $\Ain$};
\end{axis}
\end{tikzpicture}
\caption{ .}\label{fig:insilico:ISR_no_Pred}
\end{center}
\end{figure}

\begin{table}
\begin{center}
\begin{tabular}{lcccccccccc}
\toprule
%\headcol & \multicolumn{1}{c}{P3Speller}&\multicolumn{2}{c}{PolyMorph - Pred.} &\multicolumn{2}{c}{PolyMorph - No Pred.}\\
% \rulefiller\cmidrule(r){2-2} \cmidrule(r){3-4}\cmidrule(r){5-6}
%\headcol Lang&Any dataset&$\Aout$&$\Ain$&$\Aout$&$\Ain$\\
\headcol & \multicolumn{2}{c}{P3S}& \multicolumn{3}{c}{PM - Pred.} & \multicolumn{3}{c}{PM - No Pred.}\\
 \rulefiller\cmidrule(r){2-3} \cmidrule(r){4-6}\cmidrule(r){7-9}
\headcol Lang&Any&$|\nrows*\ncols|$&$\Aout$&$\Ain$&$\max{|\nrows*\ncols|}$&$\Aout$&$\Ain$&$\max{|\nrows*\ncols|}$\\
\midrule
\English&$12.00$&$6\times 6$&$11.70$&$12.81$&$7\times 6$&$10.58$&$10.55$&$6\times 6$\\
\rowcol \German&$12.00$&$6\times 6$&$11.34$&$12.77$&$7\times 6$&$10.41$&$10.40$&$6\times 6$\\
\French&$12.00$&$6\times 6$&$11.47$&$12.85$&$7\times 6$&$10.35$&$10.38$&$6\times 6$\\
\rowcol \Italian&$12.00$&$6\times 6$&$11.40$&$12.77$&$7\times 6$&$10.30$&$10.31$&$6\times 6$\\
\Finnish&$12.00$&$6\times 6$&$10.81$&$12.48$&$7\times 6$&$9.78$&$9.78$&$6\times 6$\\
\rowcol \Hungarian&$12.00$&$6\times 6$&$11.18$&$11.80$&$7\times 6$&$10.40$&$10.35$&$6\times 6$\\
\ItalianC&$12.00$&$6\times 6$&$10.66$&$11.44$&$6\times 6$&$9.92$&$9.92$&$6\times 5$\\
\bottomrule
\end{tabular}
\caption{Intensifications per Selection and Repetition (ISR)  \emph{in-silico}. 
The presence of the prediction symbols in the selection matrix may increase the number of rows $\nrows$. 
However, whenever the sentence to be spelt is not contained in the KB
the ISR of PolyMorph is smaller than that of P3Speller. 
The data observed when we disabled predictions 
(i.e. PM - No Pred.) highlight the advantage of using PolyMorph over P3Speller in term of intensifications required to 
spell a sentence.}\label{table:ISR} 
\end{center}
\end{table}

\begin{table}
\begin{center}
%\caption{PolyMorph mean characters per selections in \emph{in-silico}.}\label{table:charsel}
%\end{center}
%\end{table}
%\begin{table}
%\begin{center}
\subfloat[Mean output characters per minute\label{table:charmin}]{
\begin{tabular}{lccccccccc}
\toprule
\headcol & \multicolumn{1}{c}{P3S}& \multicolumn{2}{c}{PM - Pred.} & \multicolumn{2}{c}{PM - No Pred.}\\
 \rulefiller\cmidrule(r){2-2} \cmidrule(r){3-4}\cmidrule(r){5-6}
\headcol Lang&Any&$\Aout$&$\Ain$&$\Aout$&$\Ain$\\
\midrule
\English&$1.43$&$2.66$&$6.08$&$1.75$&$1.76$\\
\rowcol \German&$1.43$&$2.84$&$7.05$&$1.9$&$1.92$\\
\French&$1.43$&$2.8$&$6.41$&$1.82$&$1.82$\\
\rowcol \Italian&$1.43$&$2.66$&$6.36$&$1.83$&$1.82$\\
\Finnish&$1.43$&$2.74$&$7.55$&$2.07$&$1.89$\\
\rowcol \Hungarian&$1.43$&$3.62$&$6.23$&$1.89$&$1.86$\\
\ItalianC&$1.43$&$2.67$&$4.95$&$1.86$&$1.86$\\
\bottomrule
\end{tabular}}\hskip5mm
%\subfloat[Mean characters per selections\label{table:charsel}]{
\subfloat[Mean selections per minute\label{table:selmin}]{
\begin{tabular}{lccccccccc}
\toprule
\headcol & \multicolumn{1}{c}{P3S}& \multicolumn{2}{c}{PM - Pred.} & \multicolumn{2}{c}{PM - No Pred.}\\
 \rulefiller\cmidrule(r){2-2} \cmidrule(r){3-4}\cmidrule(r){5-6}
\headcol Lang&Any&$\Aout$&$\Ain$&$\Aout$&$\Ain$\\
\midrule
%\English&$1.00$&$2.12$&$5.20$&$1.10$&$1.10$\\
%\rowcol \German&$1.00$&$2.22$&$6.01$&$1.18$&$1.18$\\
%\French&$1.00$&$2.20$&$5.50$&$1.12$&$1.12$\\
%\rowcol \Italian&$1.00$&$2.09$&$5.43$&$1.12$&$1.12$\\
%\Finnish&$1.00$&$2.07$&$6.33$&$1.21$&$1.22$\\
%\rowcol \Hungarian&$1.00$&$2.80$&$5.01$&$1.17$&$1.17$\\
%\ItalianC&$1.00$&$2.00$&$3.90$&$1.10$&$1.10$\\
\English&$1.43$&$1.25$&$1.17$&$1.60$&$1.60$\\
\rowcol\German&$1.43$&$1.28$&$1.17$&$1.62$&$1.62$\\
\French&$1.43$&$1.27$&$1.17$&$1.62$&$1.62$\\
\rowcol\Italian&$1.43$&$1.27$&$1.17$&$1.63$&$1.63$\\
\Finnish&$1.43$&$1.32$&$1.19$&$1.71$&$1.55$\\
\rowcol\Hungarian&$1.43$&$1.29$&$1.24$&$1.63$&$1.59$\\
\ItalianC&$1.43$&$1.34$&$1.27$&$1.68$&$1.68$\\
\bottomrule
\end{tabular}}
\caption{Mean output characters per minute (OCM) and selections per minute (SM) in \emph{in-silico}.}\label{table:charselmin}
\end{center}
\end{table}


\begin{figure}
\begin{center}
\begin{tikzpicture}[scale=0.80]
\begin{axis}
[
width=18cm,
height=6.5cm,
ymajorgrids,
ybar,
%ymode = log,
xlabel = Language,
nodes near coords, 
every node near coord/.append style={rotate=-45, anchor=south east},
%symbolic x coords={Danish,English,Finnish,French,German,Hungarian,Italian},
%xtick={Danish,English,Finnish,French,German,Hungarian,Italian},
symbolic x coords={English,German,French,Italian,Finnish,Hungarian,{Italian Curated}},
xtick={English,German,French,Italian,Finnish,Hungarian,{Italian Curated}},
xticklabels={\English,\German,\French,\Italian,\Finnish,\Hungarian,\ItalianC},
ylabel = {Output Characters per Minute},
ymin = 0,
ymax=9.3,
%ymax=2600,     
%y unit=\si{\second},
%max space between ticks=30pt, 
%ytick={700,1400,2100},
legend columns=-1,
legend style={/tikz/every even column/.append style={column sep=0.3cm},at={(0.5,-0.3)}, anchor=north},
point meta=rawy,
]
\addplot[P3SpellerColor,fill=P3SpellerColor] table[y=CPM_P3S] from \insilicodata;
\addlegendentry{P3Speller};
\addplot[nKBColor,fill=nKBColor] table[y=CPM_nKB] from \insilicodata;
\addlegendentry{PolyMorph - $\Aout$};
\addplot[KBColor,fill=KBColor] table[y=CPM_KB] from \insilicodata;
\addlegendentry{PolyMorph - $\Ain$};
\end{axis}
\end{tikzpicture}
\caption{Mean output characters per minute in \emph{in-silico}.}\label{fig:insilico:spelling_time1}
\end{center}
\end{figure}


\begin{figure}
\begin{center}
\begin{tikzpicture}[scale=0.80]
\begin{axis}
[
width=18cm,
height=6cm,
ymajorgrids,
ybar,
%ymode = log,
xlabel = Language,
nodes near coords, 
every node near coord/.append style={rotate=-70, anchor=east},
%symbolic x coords={Danish,English,Finnish,French,German,Hungarian,Italian},
%xtick={Danish,English,Finnish,French,German,Hungarian,Italian},
symbolic x coords={English,German,French,Italian,Finnish,Hungarian,{Italian Curated}},
xtick={English,German,French,Italian,Finnish,Hungarian,{Italian Curated}},
xticklabels={\English,\German,\French,\Italian,\Finnish,\Hungarian,\ItalianC},
ylabel = {Output Characters per Minute},
ymin = 0,
ymax=3,
%ymax=2600,     
%y unit=\si{\second},
%max space between ticks=30pt, 
%ytick={700,1400,2100},
legend columns=-1,
legend style={/tikz/every even column/.append style={column sep=0.3cm},at={(0.5,-0.3)}, anchor=north},
point meta=rawy,
]
\addplot[P3SpellerColor,fill=P3SpellerColor] table[y=CPM_P3S] from \insilicodatanohints;
\addlegendentry{P3Speller};
\addplot[nKBColor,fill=nKBColor] table[y=CPM_nKB] from \insilicodatanohints;
\addlegendentry{PolyMorph - $\Aout$};
\addplot[KBColor,fill=KBColor] table[y=CPM_KB] from \insilicodatanohints;
\addlegendentry{PolyMorph - $\Ain$};
\end{axis}
\end{tikzpicture}
\caption{Mean output characters per minute in \emph{in-silico} when predictions are disabled.}\label{fig:insilico:spelling_time1_no_hints}
\end{center}
\end{figure}


%\begin{figure}[!h]
%\centering
%%\includegraphics[width=\textwidth]{ISC.pdf}
%\resizebox{0.90\textwidth}{!}{\input{ISC.tex}}
%\caption{ .}\label{fig:insilico:ISR_vs_OCS}
%\end{figure}


==> results.tex <==
%!TEX root = main.tex

\subsection{\emph{In-vivo} Analysis}

%\subsection{Time needed to spell the sentence}
%
%When analyzed the time needed to spell the sentence A using PolyMorph and P3Speller the results show that there was a significant effect of system 
%$F_{(1; 9)} = 92.52$; $P <0.0009$. According to post-hoc tests, there is a significant difference between the time required by PolyMorph to spell sentence A for 
%the $1^\textrm{st}$ time versus that needed by P3Speller ($t_{(9)} =9.37$; $P<0.0009$). Furthermore, the needed time by PolyMorph to spell sentence A for the $2^\textrm{nd}$ time was 
%lower compared with the time needed by P3Speller ($t_{(9)} = 9.97$; $P< 0.0009$). Finally, PolyMorph reduced significantly the time of the $2^\textrm{nd}$ spelling with 
%respect to the $1^\textrm{st}$ spelling of the same sentences ($t_{(9)} =5.35$; $P<0.0009$). These data are shown in Fig.~\ref{fig:spelling_time1} and in Tab 2.
%
%\pgfplotstableread{
%Subject	P1A P2A P1B P2B P3Speller P1M P2M
%1       213.13  154.4   332.13  154.38  549.13  272.63  154.38
%2       483.38  274.4   586.13  274.38  1292.63        534.755 274.38
%3       336.13  244.4   522.63  244.38  1298.13        429.38  244.38
%4       500.13  364.4   776.63  364.38  1778.63        638.38  364.38
%5       356.63  259.4   554.38  363.13  1570.63        455.505 311.255
%6       367.5   154.4   451.13  216.13  1289.25        409.315 185.255
%7       349.88  199.4   427.38  199.38  986.25  388.63  199.38
%8       315.63  275.3   490.88  229.38  894.13  403.255 252.315
%9       377.13  322.3   586.13  274.38  1484.13        481.63  298.315
%10      315.63  269.8   649.63  229.38  1205.13        482.63  249.565
%
%}\timetable
%

%\pgfplotsset{unit code/.code={\si{#1}}}
%
%\begin{figure}
%\begin{center}
%\begin{tikzpicture}[scale=0.70]
%\begin{axis}
%[
%width=22cm,
%height=6cm,
%ymajorgrids,
%ybar,
%%ymode = log,
%xlabel = Subject,
%nodes near coords, 
%every node near coord/.append style={rotate=45, anchor=south west},
%symbolic x coords={1,2,3,4,5,6,7,8,9,10},
%xtick={1,2,3,4,5,6,7,8,9,10},
%ylabel = {Time},
%ymin = 0,
%%ymax=6000,
%ymax=2600,     
%y unit=\si{\second},
%%max space between ticks=30pt, 
%ytick={700,1400,2100},
%legend columns=-1,
%legend style={/tikz/every even column/.append style={column sep=0.3cm},at={(0.5,-0.4)}, anchor=north},
%point meta=rawy,
%]
%%\addplot table[y =P3Speller] from \timetable;
%\addplot[P3SpellerBorderColor,fill=P3SpellerColor] table[y =P3Speller] from \timetable;
%\addlegendentry{P3Speller};
%%\addplot table[y =P1M] from \timetable;
%\addplot[P1MBorderColor,fill=P1MColor] table[y =P1M] from \timetable;
%\addlegendentry{$1^\textrm{st}$ PolyMorph spelling};
%%\addplot table[y =P2M] from \timetable;
%\addplot[P2MBorderColor,fill=P2MColor] table[y =P2M] from \timetable;
%\addlegendentry{$2^\textrm{nd}$ PolyMorph spelling};
%\end{axis}
%\end{tikzpicture}
%%
%%\begin{tikzpicture}[scale=0.65]     
%%        \begin{axis}[    
%%            width=20cm,
%%            xbar,                                 
%%            xtick={0,300,...,2000},    
%%            xmin=1,
%%            xmax=2000,        
%%            xmajorgrids,
%%            nodes near coords, nodes near coords align={horizontal},
%%%            every node near coord/.append style={
%%%                append after command={
%%%                    node[anchor=east] {sec}
%%%                 }
%%%            }, 
%%            symbolic y coords={10,9,8,7,6,5,4,3,2,1},
%%            ylabel={Subject},
%%            xlabel={Time (sec)},
%%            %y label style={at={(-0.1,0.5)}},
%%            enlarge x limits={abs=0},
%%            reverse legend,
%%        ]
%%        \addplot table [x=P2M, y=Subject] {\timetable};
%%        %\addplot[P2MBorderColor,fill=P2MColor] table [x=P2M, y=Subject] {\timetable};
%%        \addlegendentry{PolyMorph $2^\textrm{nd}$ spelling};
%%        %\addplot[P1MBorderColor,fill=P1MColor] table [x=P1M, y=Subject] {\timetable};
%%        \addplot table [x=P1M, y=Subject] {\timetable};
%%        \addlegendentry{PolyMoprh $1^\textrm{st}$ spelling};
%%        %\addplot[P3SpellerBorderColor,fill=P3SpellerColor] table [x=P3Speller, y=Subject] {\timetable};
%%        \addplot table [x=P3Speller, y=Subject] {\timetable};
%%        \addlegendentry{P3Speller};
%%        \end{axis}
%%\end{tikzpicture}
%\caption{Target spelling time. The times reported for PolyMorph are the averages of the times spent in spelling 
%each of the two target sequences. Those associated to P3Speller refer to the spelling of the only target sentence A. 
%All the times %(in sec) %is expressed in seconds and 
%account both the selection of periods and any misspelling correction.}\label{fig:spelling_time1}
%\end{center}
%\end{figure}
%
%%\begin{figure}
%%\caption{Time needed to spell the sentences (in sec) (including correction of errors and point). Within- subject comparison between writing sentences with PolyMorph for first time (black) and writing the  sentences with the P3Speller (gray).}\label{fig:spelling_time2}
%%\end{figure}
%%
%%\begin{figure}
%%\caption{Time needed to spell the sentences (in sec) (including correction of errors and point). Within- subject comparison between writing sentences with PolyMorph for second time (black) and writing the  sentences with P3Speller (gray).}\label{fig:spelling_time3}
%%\end{figure}
%
%Moreover, the results of rmANOVA showed a significant interaction between two main factors, namely spelling system and sentence spelling ($F_{(1; 9)} = 25.23$; $P=.001$). 
%Post-hoc comparison revealed  that the time required to spell sentence A by using PolyMorph for the $1^\textrm{st}$ time is lower than that demanded by sentence B ($t_{(9)} = 9.61$; $P<0.0009$). 
%PolyMorph also decreased the time spent to complete sentence A for the $2^\textrm{nd}$ time compared with that of the $1^\textrm{st}$ time ($t_{(9)} = 5.35$; $P<0.0005$) as well the time of the $2^\textrm{nd}$ 
%spelling of sentence B with respect to the $1^\textrm{st}$ spelling of the same sentence ($t_{(9)} = 10.73$; $P<0.0009$) (see Fig. XX and Tab. 2).
%
%\begin{figure}
%\begin{center}
%\begin{tikzpicture}[scale=0.70]
%\begin{axis}
%[
%width=22cm,
%height=6cm,
%ymajorgrids,
%ybar,
%%ymode = log,
%xlabel = Subject,
%nodes near coords, 
%every node near coord/.append style={rotate=45, anchor=south west},
%symbolic x coords={1,2,3,4,5,6,7,8,9,10},
%xtick={1,2,3,4,5,6,7,8,9,10},
%ylabel = {Time},
%ymin = 0,
%%ymax=6000,
%ymax=2600,     
%y unit=\si{\second},
%%max space between ticks=30pt, 
%ytick={700,1400,2100},
%legend columns=-1,
%legend style={/tikz/every even column/.append style={column sep=0.3cm},at={(0.5,-0.4)}, anchor=north},
%point meta=rawy,
%]
%%\addplot table[y =P3Speller] from \timetable;
%\addplot[P3SpellerBorderColor,fill=P3SpellerColor] table[y =P3Speller] from \timetable;
%\addlegendentry{P3Speller};
%%\addplot table[y =P1A] from \timetable;
%\addplot[P1MBorderColor,fill=P1MColor] table[y =P1M] from \timetable;
%\addlegendentry{$1^\textrm{st}$ PolyMorph spelling};
%%\addplot table[y =P2A] from \timetable;
%\addplot[P2MBorderColor,fill=P2MColor] table[y =P2M] from \timetable;
%\addlegendentry{$2^\textrm{nd}$ PolyMorph spelling};
%\end{axis}
%\end{tikzpicture}
%\caption{Spelling time required by the target sentence A. All the values %(in sec) %is expressed in seconds and 
%accounts the selection of period and misspelling corrections.}\label{fig:spelling_time4}
%\end{center}
%\end{figure}
%
%\begin{figure}
%\begin{center}
%\begin{tikzpicture}[scale=0.70]
%\begin{axis}
%[
%width=22cm,
%height=6cm,
%ymajorgrids,
%ybar,
%%ymode = log,
%xlabel = Subject,
%nodes near coords, 
%every node near coord/.append style={rotate=45, anchor=south west},
%symbolic x coords={1,2,3,4,5,6,7,8,9,10},
%xtick={1,2,3,4,5,6,7,8,9,10},
%ylabel = {Time},
%ymin = 0,
%%ymax=6000,
%ymax=900,     
%y unit=\si{\second},
%%max space between ticks=30pt, 
%ytick={225,450,675},
%legend columns=-1,
%legend style={/tikz/every even column/.append style={column sep=0.3cm},at={(0.5,-0.4)}, anchor=north},
%point meta=rawy,
%]
%%\addplot table[y =P3Speller] from \timetable;
%%\addplot[P3SpellerBorderColor,fill=P3SpellerColor] table[y =P3Speller] from \timetable;
%%\addlegendentry{P3Speller};
%%\addplot table[y =P1B] from \timetable;
%\addplot[P1MBorderColor,fill=P1MColor] table[y =P1M] from \timetable;
%\addlegendentry{$1^\textrm{st}$ PolyMorph spelling};
%%\addplot table[y =P2B] from \timetable;
%\addplot[P2MBorderColor,fill=P2MColor] table[y =P2M] from \timetable;
%\addlegendentry{$2^\textrm{nd}$ PolyMorph spelling};
%\end{axis}
%\end{tikzpicture}
%
%\caption{Spelling time for the sentence B. All the values %(in sec) %is expressed in seconds and 
%accounts the selection of period and misspelling corrections.}\label{fig:spelling_time5}
%\end{center}
%\end{figure}
%
%\begin{figure}
%\begin{center}
%\begin{tikzpicture}[scale=0.70]
%\begin{axis}
%[
%width=19cm,
%height=6cm,
%ymajorgrids,
%ybar,
%%ymode = log,
%xlabel = Subject,
%nodes near coords, 
%every node near coord/.append style={rotate=-45, anchor=south east},
%symbolic x coords={1,2,3,4,5,6,7,8,9,10},
%xtick={1,2,3,4,5,6,7,8,9,10},
%ylabel = {Time},
%ymin = 0,
%%ymax=6000,
%ymax=1100,     
%y unit=\si{\second},
%%max space between ticks=30pt, 
%ytick={300,600,900},
%legend columns=-1,
%legend style={/tikz/every even column/.append style={column sep=0.3cm},at={(0.5,-0.4)}, anchor=north},
%point meta=rawy,
%]
%\addplot[P1ABorderColor,fill=P1AColor] table[y =P1A] from \timetable;
%\addlegendentry{Sentence $A$};
%\addplot[P1BBorderColor,fill=P1BColor] table[y =P1B] from \timetable;
%\addlegendentry{Sentence $B$};
%\end{axis}
%\end{tikzpicture}
%
%\caption{Time required to spell a sentence for the first time. All the values %(in sec) %is expressed in seconds and 
%accounts the selection of period and misspelling corrections.}\label{fig:spelling_time6}
%\end{center}
%\end{figure}

\pgfplotstableread{
Subject	P1A	P2A	P1B	P2B P3Speller P1M P2M
1	0.0	0.0	0.0	0.0	0.0	0.0	0.0
2	0.11	0.0	0.0	0.0	0.07	0.05	0.0
3	0.0	0.0	0.0	0.0	0.13	0.0	0.0
4	0.0	0.0	0.0	0.0	0.07	0.0	0.0
5	0.0	0.0	0.0	0.14	0.17	0.0	0.08
6	0.17	0.0	0.13	0.14	0.28	0.15	0.08
7	0.11	0.0	0.0	0.0	0.1	0.05	0.0
8	0.0	0.0	0.0	0.0	0.0	0.0	0.0
9	0.0	0.0	0.0	0.0	0.13	0.0	0.0
10	0.0	0.0	0.13	0.0	0.13	0.09	0.0

}\vivoerrorseltable

%\pgfplotstableread{
%Subject	P1A	P2A	P1B	P2B P3Speller P1M P2M
%1	0.0	0.0	0.0	0.0	0.0	0.0	0.0
%2	0.04	0.0	0.0	0.0	0.09	0.02	0.0
%3	0.0	0.0	0.0	0.0	0.17	0.0	0.0
%4	0.0	0.0	0.0	0.0	0.09	0.0	0.0
%5	0.0	0.0	0.0	0.04	0.26	0.0	0.02
%6	0.09	0.0	0.09	0.04	0.65	0.09	0.02
%7	0.04	0.0	0.0	0.0	0.13	0.02	0.0
%8	0.0	0.0	0.0	0.0	0.0	0.0	0.0
%9	0.0	0.0	0.0	0.0	0.17	0.0	0.0
%10	0.0	0.0	0.09	0.0	0.17	0.04	0.0
%
%
%}\vivoerrorchartable
%
%
%\begin{figure}
%\begin{center}
%\begin{tikzpicture}[scale=0.70]
%\begin{axis}
%[
%width=22cm,
%height=6cm,
%ymajorgrids,
%ybar,
%%ymode = log,
%xlabel = Subject,
%nodes near coords, 
%every node near coord/.append style={rotate=45, anchor=south west},
%symbolic x coords={1,2,3,4,5,6,7,8,9,10},
%xtick={1,2,3,4,5,6,7,8,9,10},
%ylabel = {Errors/Character (\%)},
%ymin = 0,
%%ymax=6000,
%ymax=0.8,     
%%y unit=\si{\second},
%%max space between ticks=30pt, 
%point meta={y*100},
%nodes near coords={\pgfmathprintnumber\pgfplotspointmeta\%},
%ytick={0.25,0.5,0.75},
%yticklabel={\pgfmathparse{\tick*100}\pgfmathprintnumber{\pgfmathresult}\%},
%legend columns=-1,
%legend style={/tikz/every even column/.append style={column sep=0.3cm},at={(0.5,-0.4)}, anchor=north}
%]
%%\addplot table[y =P3Speller] from \vivoerrorchartable;
%\addplot[P3SpellerBorderColor,fill=P3SpellerColor] table[y =P3Speller] from \vivoerrorchartable;
%\addlegendentry{P3Speller};
%%\addplot table[y =P1B] from \vivoerrorchartable;
%\addplot[P1MBorderColor,fill=P1MColor] table[y =P1B] from \vivoerrorchartable;
%\addlegendentry{$1^\textrm{st}$ PolyMorph spelling};
%%\addplot table[y =P2B] from \vivoerrorchartable;
%\addplot[P2MBorderColor,fill=P2MColor] table[y =P2B] from \vivoerrorchartable;
%\addlegendentry{$2^\textrm{nd}$ PolyMorph spelling};
%\end{axis}
%\end{tikzpicture}
%\caption{Errors per character. This graph exhibits the ratio between the number of errors and the number of symbols  
%that compose the target sentence. 
%The values reported for PolyMorph are the averages of the errors per character obtained by spelling 
%each of the two target sequences. Those associated to P3Speller refer to the spelling of the only target sentence A.
%}\label{fig:errors_per_char}
%\end{center}\end{figure}

%\subsection{Number of Total Intensifications}
%
%
%About the total number of intensifications (NTI) needed to spell the sentence A using PolyMorph and P3Speller,  
%ANOVA reported a significant main effect of System $F_{(1; 9)} = 84.47$; $P <0.0009$. The NTI required to spell sentence A 
%for the $1^\textrm{st}$ time with PolyMorph was lower versus that required by P3Speller ($t_{(9)} =9.04$; $P<0.0009$). Moreover, a significant 
%difference was found between the NTI needed to spell sentence A with PolyMorph for the $2^\textrm{nd}$  time when compared with 
%that required with the P3Speller ($t_{(9)} = 9.4$; $P< 0.0009$). In addition, the NTI needed to spell sentence A with PolyMorph for 
%the $2^\textrm{nd}$ time was reduced compared with the NTI needed to spell the same phrase with PolyMorph for the $1^\textrm{st}$ time 
%($t_{(9)} =5.41$; $P<0.0004$). These data are shown in Fig. XX and in Tab.3. 
%
%rmANOVA unravels a significant interaction between writing system and spelled sentence ($F_{(1; 9)} = 22.68$; $P<0.001$). 
%We found decreased NTI for PolyMorph when writing sentence A for the $1^\textrm{st}$ time with respect the NTI required when 
%writing sentence B for the $1^\textrm{st}$ time ($t_{(9)} = 5.96$; $P<0.0002$). Moreover, PolyMorph requires less NTI to spell the sentence A  for the $2^\textrm{nd}$ time 
%with respect to the $1^\textrm{st}$ time ($t_{(9)} = 5.41$; $P<0.0004$) and, analogously, the NTI needed to spell sentence B for the $2^\textrm{nd}$ time 
%is smaller than that required by $1^\textrm{st}$ time ($t_{(9)} = 8.52$; $P<0.0009$). 
%\textbf{In addition, the NTI needed to complete sentence B were lowered when using PolyMorph for the $2^\textrm{nd}$ time compared with the 
%NTI required to write the phrase A for the $1^\textrm{st}$ time ($t_{(9)} = 5.31$; $P<0.0005$)} (see Fig. XX). 

\subsubsection{Output Characters per Minutes (OCM)}

%Evaluating output characters per minute (OCM) in spelling sentence A by using both PolyMorph and P3Speller highlighted 
%significant differences within subjects ($df = 2$; $\chi^2 = 20$). 
Concerning sentence A, we observed larger OCM in both turn 1 and 2 of PolyMorph session with respect to that obtained by using P3Speller 
(Wilcoxon test: $P = 0.00195$ in both cases \textbf{?????}).
%when spelling the sentence A in turn 1 %for the $1^\textrm{st}$  time 
%%with PolyMorph with respect to OCM obtained by P3Speller 
%(Wilcoxon test: $P = 0.00195$). 
%We also found an increase of OCM for PolyMorph turn 2 of sentence A %when 
%spelling the sentence A in turn 2 %for the $2^\textrm{nd}$ time 
%with PolyMorph 
%in regard to that of P3Speller (Wilcoxon test: $P = 0.0195$). 
It was also detected 
relevant enhancement of OCM from turn 1 to turn 2 %writing the sentence 
%for the $1^\textrm{st}$ and for the $2^\textrm{nd}$ time with PolyMorph 
(Wilcoxon test: $P = 0.00195$). 

The rmANOVA showed a significant interaction between writing system and spelled sentence ($F_{(1; 9)} = 6.33$; $P=.033$). 
With regard to PolyMorph, we found a substantially increased OCM %when writing sentence A for  the$1^\textrm{st}$ time with PolyMorph compared with the OCM when 
%writing sentence B for the $1^\textrm{st}$ time 
in turn 1 of sentence A compared with the OCM of the same turn of sentence B  
($t_{(9)} = 6.69$; $P<0.0009$) and we observed an increased OCM %when writing sentence B 
%for the $2^\textrm{nd}$ time with PolyMorph with respect the OCM when writing sentence A for the $1^\textrm{st}$ time 
in turn 2 of sentence B against that of turn 1 of sentence A 
($t_{(9)} = 6.24$; $P<0.0002$). 
Finally, the OCM obtained during turn 2 is larger than that of turn 1 for both sentence A and B 
%when spelling sentence A was increased when using  PolyMorph for the $2^\textrm{nd}$ time compared with this 
%value obtained when writing the same sentence for the $1^\textrm{st}$ time 
($t_{(9)} = 4.2$; $P<0.002$ and $t_{(9)} = 9.88$; $P<0.0009$, respectively). %Finally, the OCM recorded %when spelling 
%sentence B was increased when using PolyMorph for the $2^\textrm{nd}$ time compared with the OCM obtained when writing the same 
%sentence for the $1^\textrm{st}$ time ($t_{(9)} = 9.88$; $P<0.0009$).  

%\begin{figure}
%\begin{center}
%\begin{tikzpicture}[scale=0.70]
%\begin{axis}
%[
%width=22cm,
%height=6cm,
%ymajorgrids,
%ybar,
%%ymode = log,
%xlabel = Subject,
%nodes near coords, 
%every node near coord/.append style={rotate=45, anchor=south west},
%symbolic x coords={1,2,3,4,5,6,7,8,9,10},
%xtick={1,2,3,4,5,6,7,8,9,10},
%ylabel = {Errors/Selection (\%)},
%ymin = 0,
%%ymax=6000,
%ymax=0.35,     
%%y unit=\si{\second},
%%max space between ticks=30pt, 
%point meta={y*100},
%nodes near coords={\pgfmathprintnumber\pgfplotspointmeta\%},
%ytick={0.11,0.22,0.33},
%yticklabel={\pgfmathparse{\tick*100}\pgfmathprintnumber{\pgfmathresult}\%},
%legend columns=-1,
%legend style={/tikz/every even column/.append style={column sep=0.3cm},at={(0.5,-0.4)}, anchor=north}
%]
%%\addplot table[y =P3Speller] from \vivoerrorseltable;
%\addplot[P3SpellerBorderColor,fill=P3SpellerColor] table[y =P3Speller] from \vivoerrorseltable;
%\addlegendentry{P3Speller};
%%\addplot table[y =P1B] from \vivoerrorseltable;
%\addplot[P1MBorderColor,fill=P1MColor] table[y =P1M] from \vivoerrorseltable;
%\addlegendentry{$1^\textrm{st}$ PolyMorph spelling};
%%\addplot table[y =P2B] from \vivoerrorseltable;
%\addplot[P2MBorderColor,fill=P2MColor] table[y =P2M] from \vivoerrorseltable;
%\addlegendentry{$2^\textrm{nd}$ PolyMorph spelling};
%\end{axis}
%\end{tikzpicture}
%\caption{Errors per selection. This graph exhibits the ratio between the number of errors and the number of symbols  
%selected to spell the target sentence. 
%The values reported for PolyMorph are the averages of the errors per selection obtained by spelling 
%each of the two target sequences. Those associated to P3Speller refer to the spelling of the only target sentence A. 
%}\label{fig:errors_per_selection}
%\end{center}
%\end{figure}

\pgfplotstableread{
Subject P1A     P2A     P1B     P2B     P3Speller       P1M     P2M
1       6.48    8.94    4.16    8.94    2.51    5.32    8.94
2       2.85    5.03    2.35    5.03    1.07    2.60    5.03
3       4.11    5.65    2.64    5.65    1.06    3.37    5.65
4       2.76    3.79    1.78    3.79    0.78    2.27    3.79
5       3.87    5.32    2.49    3.80    0.88    3.18    4.56
6       3.76    8.94    3.06    6.39    1.07    3.41    7.66
7       3.94    6.92    3.23    6.92    1.40    3.59    6.92
8       4.37    5.01    2.81    6.02    1.54    3.59    5.51
9       3.66    4.28    2.35    5.03    0.93    3.01    4.66
10      4.37    5.12    2.12    6.02    1.15    3.25    5.57

}\vivoOCMtable

\begin{figure}
\begin{center}
\begin{tikzpicture}[scale=0.70]
\begin{axis}
[
width=22cm,
height=6cm,
ymajorgrids,
ybar,
%ymode = log,
xlabel = Subject,
nodes near coords, 
every node near coord/.append style={rotate=-45, anchor=south east},
symbolic x coords={1,2,3,4,5,6,7,8,9,10},
xtick={1,2,3,4,5,6,7,8,9,10},
xticklabels={\subject{1},\subject{2},\subject{3},\subject{4},\subject{5},\subject{6},\subject{7},\subject{8},\subject{9},\subject{10}},
ytick={3,6,9},
ylabel = {Mean OCM},
ymin = 0,
ymax=11.5,
%ymax=0.35,     
%y unit=\si{\second},
%max space between ticks=30pt, 
%point meta={y*100},
%nodes near coords={\pgfmathprintnumber\pgfplotspointmeta\%},
%ytick={0.11,0.22,0.33},
%yticklabel={\pgfmathparse{\tick*100}\pgfmathprintnumber{\pgfmathresult}\%},
legend columns=-1,
legend style={/tikz/every even column/.append style={column sep=0.3cm},at={(0.5,-0.4)}, anchor=north}
]
%\addplot table[y =P3Speller] from \vivoerrorseltable;
\addplot[P3SpellerBorderColor,fill=P3SpellerColor] table[y =P3Speller] from \vivoOCMtable;
\addlegendentry{P3Speller};
%\addplot table[y =P1B] from \vivoerrorseltable;
\addplot[P1MBorderColor,fill=P1MColor] table[y =P1M] from \vivoOCMtable;
\addlegendentry{PolyMorph - Turn 1};
%\addplot table[y =P2B] from \vivoerrorseltable;
\addplot[P2MBorderColor,fill=P2MColor] table[y =P2M] from \vivoOCMtable;
\addlegendentry{PolyMorph - Turn 2};
\end{axis}
\end{tikzpicture}
\caption{Mean output characters per minute \emph{in-vivo}: the times reported for PolyMorph turn 1 and 2 are the means of the spelling times 
of sentence A and B in turn 1 and turn 2 respectively.}\label{fig:OCM_vivo}
\end{center}
\end{figure}

\subsubsection{Online accuracy}

The online accuracy was assessed, there were significant differences within subjects ($df = 2$; $\chi^2 = 6.87$). Post-hoc analysis show a significant enhancement of accuracy 
in both PolyMorph turn 1 and 2 of sentence A 
%when spelling the  sentence A for the $1^\textrm{st}$ time with PolyMorph 
with respect to the accuracy level obtained in P3Speller (Wilcoxon test: $P = 0.039$ and $ P = 0.074$, respectively) 
%Moreover, we observed improvement of accuracy when spelling the sentence for the $2^\textrm{nd}$ time with PolyMorph with respect to P3Speller (Wilcoxon test: P = 0.074) 
(see Tab.~\ref{table:accuracy}).
%Analogously, an improvement was observed from te

\begin{table}
\begin{center}
\subfloat[Online accuracy (AC). Data are reported in the format ``(number of correct selections)/(total number of selections)''.\label{table:accuracy}]{
\begin{tabular}{lccccc}%LLLLLL}
\toprule
\headcol & \multicolumn{3}{c}{Sentence A}& \multicolumn{2}{c}{Sentence B}\\
 \rulefiller\cmidrule(r){2-4} \cmidrule(r){5-6}
\headcol Subj &  PM $1$& PM $2$ & P3S & PM $1$ &  PM $2$ \\
\midrule
\subject{1} & $7/7$ & $5/5$ & $23/23$ & $11/11$ & $5/5$ \\
\rowcol  \subject{2}& $8/9$ & $5/5$ & $25/27$ & $11/11$ & $5/5$\\
\subject{3} & $7/7$ & $5/5$ & $27/31$ & $11/11$ & $5/5$\\
\rowcol \subject{4} & $7/7$ & $5/5$ & $25/27$ & $11/11$ & $5/5$\\
\subject{5} & $7/7$ & $5/5$ & $29/35$&  $11/11$ & $6/7$\\
\rowcol \subject{6} & $10/12$ & $5/5$ & $37/54$ &  $13/15$ & $6/7$\\
\subject{7} & $8/9$ & $5/5$ & $26/29$ &  $11/11$ & $5/5$\\
\rowcol \subject{8} & $7/7$ & $5/6$ & $23/23$ &  $11/11$ & $5/5$\\
\subject{9} & $7/7$ & $6/6$ & $27/31$ &  $11/11$ & $5/5$\\
\rowcol \subject{10} & $7/7$ & $5/5$ & $27/31$ &  $13/15$ & $6/6$\\
\midrule
\rescol Total & $75/79$ & $51/52$ & $272/311$ & 
$114/118$ & $53/55$\\
\bottomrule
\end{tabular}}
\hskip3mm
\subfloat[Errors per character (EC). Data are reported in the format ``(wrong selections)/(number of characters in the sentence)''.\label{table:errors_per_character}]{
\begin{tabular}{lccccc}%LLLLLL}
\toprule
\headcol & \multicolumn{3}{c}{Sentence A}& \multicolumn{2}{c}{Sentence B}\\
 \rulefiller\cmidrule(r){2-4} \cmidrule(r){5-6}
\headcol Subj &  PM $1$& PM $2$ & P3S & PM $1$ &  PM $2$ \\
\midrule
\subject{1} & $0/23$ & $0/23$ & $0/23$ & $0/23$ & $0/23$ \\
\rowcol \subject{2} & $1/23$ & $0/23$ & $2/23$ & $0/23$ & $0/23$\\
\subject{3} & $0/23$ & $0/23$ & $4/23$& $0/23$ & $0/23$\\
\rowcol \subject{4} & $0/23$ & $0/23$ & $2/23$ & $0/23$ & $0/23$\\
\subject{5} & $0/23$ & $0/23$ & $6/23$&  $0/23$ & $1/23$\\
\rowcol \subject{6} & $2/23$ & $0/23$ & $17/23$ &  $2/23$ & $1/23$\\
\subject{7} & $1/23$ & $0/23$ & $3/23$ &  $0/23$ & $0/23$\\
\rowcol \subject{8} & $0/23$ & $1/23$ & $0/23$ &  $0/23$ & $0/23$\\
\subject{9} & $0/23$ & $0/23$ & $4/23$ &  $0/23$ & $0/23$\\
\rowcol \subject{10} & $0/23$ & $0/23$ & $4/23$ &  $2/23$ & $0/23$\\
\midrule
\rescol Total & $4/230$ & $1/230$ & $41/230$ & 
$4/230$ & $2/230$\\
\bottomrule
\end{tabular}}
\caption{Online accuracy (AC) and errors per character (EC) for PolyMorph turn 1 (PM $1$),  PolyMorph turn 2 (PM $2$),  
and P3Speller (P3S).}
%\caption{Online accuracy (AC) for PolyMorph turn 1 (PM $1$),  PolyMorph turn 2 (PM $2$), 
%and P3Speller (P3S). Data are reported in the format ``(number of correct selections)/(total number of selections)''.}\label{table:accuracy}
\end{center}
\end{table}

\begin{table}
\begin{center}
\begin{tabular}{lccccc}%LLLLLL}
\toprule
\headcol & \multicolumn{3}{c}{Sentence A}& \multicolumn{2}{c}{Sentence B}\\
 \rulefiller\cmidrule(r){2-4} \cmidrule(r){5-6}
\headcol Subj &  PM $1$& PM $2$ & P3S & PM $1$ &  PM $2$ \\
\midrule
\subject{1}&$11.71$&$12.00$&$12.00$&$11.55$&$12.00$\\
\rowcol \subject{2}&$11.67$&$12.00$&$12.00$&$11.55$&$12.00$\\
\subject{3}&$11.71$&$12.00$&$12.00$&$11.55$&$12.00$\\
\rowcol \subject{4}&$11.71$&$12.00$&$12.00$&$11.55$&$12.00$\\
\subject{5}&$11.71$&$12.00$&$12.00$&$11.55$&$12.00$\\
\rowcol \subject{6}&$11.83$&$12.00$&$12.00$&$11.47$&$12.00$\\
\subject{7}&$11.56$&$12.00$&$12.00$&$11.55$&$12.00$\\
\rowcol \subject{8}&$11.71$&$12.00$&$12.00$&$11.55$&$12.00$\\
\subject{9}&$11.71$&$11.67$&$12.00$&$11.55$&$12.00$\\
\rowcol \subject{10}&$11.71$&$12.00$&$12.00$&$11.07$&$12.00$\\
\bottomrule
\end{tabular}
\caption{Intensifications per Selection and Repetition (ISR)}
\end{center}
\end{table}

\subsubsection{Errors per character}

Errors per each character selected were assessed. Test indicates that the distribution of results significantly differ within subjects ($df = 2$;  $\chi^2 = 14.89$). Post-hoc analysis 
exhibits a significant reduction of errors per each character in both PolyMorph turn 1 and 2 of sentence A 
%when spelling the  sentence A for the $1^\textrm{st}$ time with PolyMorph 
with respect to errors per each character 
obtained in P3Speller (Wilcoxon test: $P = 0.0078$ and $P = 0.00748$, respectively) (see Tab.~\ref{table:errors_per_character}).


